Agglomerative Token Clustering

We present Agglomerative Token Clustering (ATC), a novel token merging method that consistently outperforms previous token merging and pruning methods across image classification, image synthesis, and object detection & segmentation tasks. ATC merges clusters through bottom-up hierarchical clustering, without the introduction of extra learnable parameters. We find that ATC achieves state-of-the-art performance across all tasks, and can even perform on par with prior state-of-the-art when applied off-the-shelf, i.e. without fine-tuning. ATC is particularly effective when applied with low keep rates, where only a small fraction of tokens are kept and retaining task performance is especially difficult.

==> figures_tables/4_partial_results.tex <==
\begin{table*}[!t]
\caption{\textbf{Hard Token Merging Method Comparison with the DeiT Backbone.} We compare the hard-merging token reduction methods considered by Haurum \etal \cite{Haurum_2023_ICCV} with the proposed ATC method. All methods have been fine-tuned. Model performance is measured across keep rates, $r$, denoted in percentage of tokens kept at each reduction stage, and with the DeiT-Tiny, DeiT-Small, and DeiT-Base models. Comparison with all 13 token reduction methods considered by Haurum \etal can be found in the supplementary materials. ImageNet and NABirds performance is measured with top-1 accuracy, whereas COCO and NUS-WIDE is measured with mAP. The best performing method per column is denoted in \textbf{bold}. Note that ToMe is limited to $r\geq 50\%$.}
\label{tab:perfICCVPartial}


\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccclcccclcccclcccc}
\toprule
 & \multicolumn{4}{c}{ImageNet} &  & \multicolumn{4}{c}{NABirds} &  & \multicolumn{4}{c}{COCO} &  & \multicolumn{4}{c}{NUS-WIDE} \\ \cmidrule(lr){2-5} \cmidrule(lr){7-10} \cmidrule(lr){12-15} \cmidrule(lr){17-20}  %\midrule 
 
DeiT-T & \multicolumn{4}{c}{72.20} & & \multicolumn{4}{c}{74.16} & & \multicolumn{4}{c}{71.09} & & \multicolumn{4}{c}{59.27} \\ \midrule\midrule
$r$  (\%) & 25 & 50 & 70 & 90 &  & 25 & 50 & 70 & 90 &  & 25 & 50 & 70 & 90 &  & 25 & 50 & 70 & 90 \\\midrule

ToMe & - & 69.72 & 71.74 & 72.16 &  & - & 66.61 & 73.65 & \textbf{74.50} &  & - & 65.66 & 69.70 & \textbf{71.16} &  & - & 55.32 & 57.78 & 58.98 \\
K-Medoids & 57.50 & 65.82 & 69.90 & 71.50 &  & 44.62 & 66.52 & 72.09 & 74.04 &  & 54.08 & 64.83 & 69.09 & 71.05 &  & 49.13 & 55.92 & \textbf{58.38} & 59.07 \\
DPC-KNN & 64.56 & 69.68 &71.10 & 71.88 &  & \textbf{64.23} & 71.05 & 73.02 & 74.05 &  & 63.32 & 68.03 & 69.55 & 70.84 &  & 55.37 & 57.33 & 58.08 & 58.88 \\ \midrule

ATC$^{\text{single}}$ (ours)& 61.79& 69.93& 71.74& 72.15& & 59.27& 71.90& \textbf{73.86}& 74.18& & 60.26& 68.22& \textbf{70.19}& 70.52& & 53.36& \textbf{57.81}& 58.01& 60.19\\
ATC$^{\text{average}}$ (ours)& 66.52& 70.98& 71.83& \textbf{72.21}& & 63.96  & \textbf{72.00}& 73.72& 74.23& & \textbf{65.32}& \textbf{68.99}& 69.91& 70.48& & 56.64& 57.22& 57.88& 58.38\\
ATC$^{\text{complete}}$ (ours)& \textbf{66.69}& \textbf{71.03}& \textbf{71.87}& 72.15& & 62.96& 71.39& 73.69& 74.20& & 65.27& 68.96& 69.65& 70.47& & \textbf{56.71}& 57.28& 57.61& \textbf{60.22}\\ 
 \midrule

&&&&&&&&&&&&&&&&&&\\ \midrule



DeiT-S & \multicolumn{4}{c}{79.85} & & \multicolumn{4}{c}{80.57} & & \multicolumn{4}{c}{78.11} & & \multicolumn{4}{c}{63.23} \\ \midrule\midrule
$r$  (\%) & 25 & 50 & 70 & 90 &  & 25 & 50 & 70 & 90 &  & 25 & 50 & 70 & 90 &  & 25 & 50 & 70 & 90 \\\midrule
ToMe & - & 78.29 & 79.63 & 79.92 &  & - & 74.99 & 80.05 & \textbf{80.68} &  & - & 74.99 & 77.36 & 77.88 &  & - & 61.51 & 62.50 & 62.89 \\
K-Medoids & 68.94 & 76.44 & 78.74 & 79.73 &  & 65.28 & 76.95 & 79.75 & 80.46 &  & 66.26 & 74.15 & 76.76 & 77.94 &  & 57.78 & 61.48 & 62.47 & 63.12 \\
DPC-KNN & 75.01 & 77.95 & 78.85 & 79.54 &  & 68.77 & 74.14 & 76.70 & 78.88 &  & 72.15 & 75.70 & 77.06 & 77.74 &  & 60.78 & 62.11 & 62.67 & 62.93 \\  \midrule

ATC$^{\text{single}}$ (ours)& 73.41& 78.44& 79.58& 79.90& & 72.16& 79.18& 80.34& \textbf{80.68}& & 70.55& 75.51& 77.36& 77.94& & 59.71& 61.50& 62.58& \textbf{63.46}\\
ATC$^{\text{average}}$ (ours)& \textbf{76.42}& \textbf{79.23}& \textbf{79.82}& \textbf{79.95}& & \textbf{74.43}& \textbf{79.32}& \textbf{80.43}& 80.64& & 72.55& 76.47& 77.51& 77.95& & 60.90& 62.13& \textbf{62.93}& 63.14\\
ATC$^{\text{complete}}$ (ours)& 76.34& 79.20& 79.77& 79.90& & 73.67& 79.27& 80.37& 80.66& & \textbf{72.65}& \textbf{76.60}& \textbf{77.52}& \textbf{77.98}&& \textbf{60.96}& \textbf{62.47}& 62.85& 63.44\\ 
 \midrule

&&&&&&&&&&&&&&&&&&\\ \midrule



DeiT-B & \multicolumn{4}{c}{81.85} &  & \multicolumn{4}{c}{83.32} &  & \multicolumn{4}{c}{80.93} &  & \multicolumn{4}{c}{64.37} \\ \midrule\midrule
$r$  (\%) & 25 & 50 & 70 & 90 &  & 25 & 50 & 70 & 90 &  & 25 & 50 & 70 & 90 &  & 25 & 50 & 70 & 90 \\ \midrule
ToMe & - & 78.89 & 81.05 & 82.00 &  & - & 73.67 & 81.59 & 82.98 &  & - & 74.11 & 78.82 & 80.48 &  & - & 62.38 & \textbf{64.06} & 64.35 \\
K-Medoids & 69.12 & 76.86 & 79.98 & 81.76 &  & 57.54 & 75.29 & 80.62 & 82.57 &  & 61.79 & 73.60 & 77.58 & 80.32 &  & 56.67 & 62.18 & 63.53 & 64.35 \\
DPC-KNN & 69.40 & 75.87 & 79.06 & 81.05 &  & 58.16 & 67.36 & 72.83 & 78.29 &  & 65.99 & 73.32 & 77.03 & 79.76 &  & 58.58 & 61.39 & 62.96 & 63.87 \\ \midrule

ATC$^{\text{single}}$ (ours)& 70.00& 79.10& 81.01& \textbf{82.04}& & 64.14& 78.91& 81.79& \textbf{83.12}& & 66.76& 75.49& \textbf{79.69}& \textbf{80.70}& & 58.79& 61.51& 63.93& \textbf{64.82}\\
ATC$^{\text{average}}$ (ours)& \textbf{73.81}& \textbf{79.79}& 81.10& 81.76& & \textbf{67.55}& \textbf{79.07}& \textbf{81.88}& 83.10& & \textbf{68.61}& 75.87& 79.57& 80.65& & \textbf{59.74}& \textbf{63.02}& 64.02& 64.42\\
ATC$^{\text{complete}}$ (ours)& 73.80& 79.75& \textbf{81.15}& 82.03& & 66.14& 78.44& 81.67& 83.08& & 68.46& \textbf{76.05}& 79.40& 80.67& & 59.64& 62.91& 63.95& 64.77\\\bottomrule

\end{tabular}%
}
\end{table*}
